Self-Support Few-Shot Semantic Segmentation

Existing few-shot segmentation methods have achieved great progress based on the support-query matching framework. But they still heavily suffer from the limited coverage of intra-class variations from the few-shot supports provided. Motivated by the simple Gestalt principle that pixels belonging to the same object are more similar than those to different objects of same class, we propose a novel self-support matching strategy to alleviate this problem, which uses query prototypes to match query features, where the query prototypes are collected from high-confidence query predictions. This strategy can effectively capture the consistent underlying characteristics of the query objects, and thus fittingly match query features. We also propose an adaptive self-support background prototype generation module and self-support loss to further facilitate the self-support matching procedure. Our self-support network substantially improves the prototype quality, benefits more improvement from stronger backbones and more supports, and achieves SOTA on multiple datasets. Codes are at \url{https://github.com/fanq15/SSP}.

==> old-1-introduction-old.tex <==
\begin{comment}

\fancomment{introduction is messy}
\fancomment{Follow CK's definition of self-support prototype and maybe shorten it to self-prototype (but it misses the important information of support)? Not sure. I think self-support prototype is better and accurate.}

Definition and names:
\begin{itemize}
    \item support prototype v.s. self-support prototype
    \item matching v.s. self-support matching
    \item self-support module (SSM)
    \item pointwise similarity-sensitive background prototype \fancomment{we need better name}
    \item self-support loss/supervision (SSL/SSS)
\end{itemize}


\fancomment{Follow Wing's suggestion to introduce our method: the core problem of FSS is that limited by the data volume in few-shot learning, there is a large gap between support and query features caused by the data diversity. All other methods are trying to find the solution.}

\end{comment}


% 1. Introduce FSS
Semantic segmentation has achieved remarkable advances tapping into deep learning networks~\cite{Goodfellow-et-al-2016,krizhevsky2012imagenet,he2016deep} and large-scale datasets such as~\cite{deng2009imagenet,benenson2019large,zhou2017scene}. However, current high performing semantic segmentation methods rely heavily on laborious pixel-level annotations, % 
which has expedited the recent development of %encourage the emergence and booming development of 
few-shot semantic segmentation (FSS).
% It greatly promotes the development of few-shot semantic segmentation (FSS), which 

Few-shot semantic segmentation aims to segment arbitrary novel classes using only a few support samples. The mainstream paradigm is the support-query matching network~\cite{dong2018few}, whic
%to refrain from overfitting problem. It
applies a siamese network~\cite{koch2015siamese} to match support prototypes and query features, so as to learn a general matching metric that effectively generalizes from the training classes to the novel classes.

\fancomment{
The dilemma for few-shot semantic segmentation is that the support images are limited and fixed (usually $\{1,3,5,10\}$ supports per class), while the query images are theoretically infinite and arbitrary. The few-shot supports fail to cover the potential object appearance variations of the target class in query images, regardless of the support quality.
Thus there is a potentially large appearance discrepancy between support and query images.
This is clearly caused by the inherent data scarcity and diversity, two long standing issues in few-shot learning.
As shown in Figure~\ref{fig:teaser}, 
the cats in the query and support images are very different in color, parts and scales,
while FSS requires the pertinent model to segment the black cat supported by the highly distinctive garfield cat head.
%Previous methods heavily suffer the \ourproblem problem.
Previous methods aggregate the garfield cat features to generate the support prototype for the cat class, and then directly utilize the cat prototype to match query features of the black cat. Undoubtedly, it is hard to correctly match these cats with high appearance differences and thus the matching results are inferior as expected, where only the black cat head can be correctly segmented.
}

\fancomment{
The appearance discrepancy problem causes the inferior performance.
Existing methods try to solve the problem by making full use of the limited supports, such as proposing better matching mechanism~\cite{siam2020weakly,liu2020dynamic,yang2020brinet,wang2020few,zhang2019pyramid,he2021progressive,zhuge2021deep} or generating representative prototypes~\cite{siam2019amp,li2021adaptive,ouyang2020self,liu2020part,yang2021mining,kim2021uncertainty,nguyen2019feature,yang2020prototype,zhang2019canet,gairola2020simpropnet}. Despite their success, they are still narrowly bounded by the provided few-shot supports.
Recently, some methods~\cite{liu2020ppnet,yang2021mining} try to break the few-shot support limit by introducing extra unlabeled images to prototype generation or modeling training.
But the extra images still cannot guarantee the appearance consistency between support and query images.
%improve the matching paradigm from various aspects, \eg, matching mechanism~\cite{siam2020weakly,liu2020dynamic,yang2020brinet,wang2020few,zhang2019pyramid,he2021progressive,zhuge2021deep}, training supervision~\cite{boudiaf2021few,wang2019panet,zhang2021self,liu2020crnet,liu2021learning} and support generation~\cite{siam2019amp,li2021adaptive,ouyang2020self,liu2020part,yang2021mining,kim2021uncertainty,nguyen2019feature,yang2020prototype,zhang2019canet,gairola2020simpropnet}. 
}

\begin{comment}

\fancomment{
Although previous methods cannot fundamentally solve the appearance discrepancy problem, they still provide some reliable predictions on those query regions which have high appearance or semantic similarity with supports, \eg, the lack cat head can be correctly segmented in Figure~\ref{fig:teaser}.
}
\end{comment}

\fancomment{
Our solution is motivated by the intuition of pixels belonging to the same object are more similar than those to different objects, which has been summarized as Gestalt law~\cite{gestalt}.
We propose a novel query-query matching concept to solve the appearance discrepancy problem: use query prototypes to match query features, or in other words, use the query feature to self-support itself. We thus call the query prototype as self-support prototype because of its self-matching property. The self-matching among pixels in the same image guarantees the high appearance consistency between self-support prototype and query images. As shown in Table~\ref{table:teaser-1}, 
}


\begin{comment}

People try to learn a general metric to use the few-shot supports to match the infinite query images,
two ways: 1. learn a good and robust metric
2. generate more representative support prototype
However, these methods are still problemetic,
In the feature space, we can not learn a perfect metric to correctly classify each query into the right support class
We also can not generate perfect support prototype to correctly match every query images
we can not make sure that support and query objects is similar, especially for the limited support images,
if we have enough images, we can train a good metric to correctly classify each image, the classifier weight is the learned supports, which is trained on numerous images to fit the classification
However, we only have a few supports, 
The fully-supervised classifier can classify black dog and white dog as the same class, but for the few-shot segmentation, it is hard to use a white dog to match a black dog. It is more probably to support can only segment some parts of the dog with high semantic similarity, but for other regions, like the body, it is hard to segment the body using the white dog support.
It is impossible and illness to use limited supports to cover all variations of the query objects.
Let's check how FSS works.
What the model can do is to cover only those regions with high semantic similarity and misclassify other regions.
Now, we have those high-confidence regions, and those regions with high uncertainty, how can we solve it.
The essence is to 

$Q_{pred} = M(S_{prototype}, Q_{feature})$

\begin{equation}
    Q_{pred} = M(S_{prototype}, Q_{feature})
\end{equation}

\begin{equation}
    Q_{pred} = Q^{high}_{pred} + Q^{low}_{pred}
\end{equation}

\begin{equation}
    Q = M(Q^{high}_{prototype}, Q_{feature})
\end{equation}

\begin{equation}
    Q^{hight}_{prototype} = Q^{high}_{pred} * Q_{feature}
\end{equation}

\end{comment}


%Most FSS works have then contributed to improve the matching paradigm from various aspects, \eg, matching mechanism~\cite{siam2020weakly,liu2020dynamic,yang2020brinet,wang2020few,zhang2019pyramid,he2021progressive,zhuge2021deep}, training supervision~\cite{boudiaf2021few,wang2019panet,zhang2021self,liu2020crnet,liu2021learning} and support generation~\cite{siam2019amp,li2021adaptive,ouyang2020self,liu2020part,yang2021mining,kim2021uncertainty,nguyen2019feature,yang2020prototype,zhang2019canet,gairola2020simpropnet}. 


\begin{comment}

\begin{figure}
\centering
%\fbox{\rule{0pt}{2.0in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=1.0\linewidth]{figure/teaser-3.pdf}
\vspace{-0.3in}
\caption{Comparison between (a) the traditional prototype-based matching network and (b) our self-support prototype-based matching network, which aggregates query features to generate self-support prototypes for support-query matching.
We also present (c) the intra-class appearance variations for the cat class.}
\label{fig:teaser}
\vspace{-0.2in}
\end{figure}

\end{comment}


\begin{figure}[!t]
\centering
%\fbox{\rule{0pt}{2.0in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=1.0\linewidth]{figure/teaser-new.pdf}
\vspace{-0.2in}
\caption{The \textit{left} image illustrates the core idea of our self-support matching. We use the initial query mask prediction to collect query features in high-confidence regions and then use the generated \textbf{query prototype} to perform \textbf{self-matching} with \textbf{query features}.
The \textit{right} image illustrates that our self-support matching is fundamentally distinct from other methods.}

\label{fig:teaser}
\end{figure}

\begin{comment}

% 2. Introduce problem and previous works
Despite their success, 
existing few-shot segmentation methods heavily suffer from 
%the intra-class appearance discrepancy problem between query and support images.
the narrow coverage of intra-class variations by few-shot supports,
which fail to sufficiently cover the potential object appearance variations of the target class in query images, regardless of the support quality.
%the narrow coverage of intra-class variations by few-shot supports, 
%which fail to sufficiently cover the potential object appearance variations of the target class, regardless of the support quality.
%they rarely explore the inherent {\it inconsistent matching}  (\fancomment{we need a better problem name, the following description is correct.}) problem in FSS: objects in query and support images are highly different and therefore hard to match them.
This is clearly caused by the inherent data scarcity and diversity, two long standing issues in few-shot learning.
As shown in Figure~\ref{fig:teaser}, 
the cats in the query and support images are very different in color, parts and scales,
while FSS requires the pertinent model to segment the black cat supported by the highly distinctive garfield cat head.
%Previous methods heavily suffer the \ourproblem problem.
Previous methods aggregate the garfield cat features to generate the support prototype for the cat class, and then directly utilize the cat prototype to match query features of the black cat. Undoubtedly, it is hard to correctly match these cats with high appearance differences and thus the matching results are inferior as expected, where only the black cat head can be correctly segmented.
%Previous methods aggregate support features to generate the support prototype and directly utilize them to match query features. It is hard to correctly segment the whole black cat using the prototype generated by the white cat head.

\end{comment}


% high appearance variance 
% the few-shot support can not cover all appearance variations
% intra-class variation
% by pei: limited coverage of intra-class variations by few shot supports
%by pei: regardless of the quality of the support images, for an object class, the provided few-shot support images cannot cover fully the potential appearance variations of objects in this class.
%This paper proposes to solve the problem by introducing query features into support prototypes, or in other words, the query feature can self-support itself.
%This new idea redefines the prototype generation where so far only support features have been used to match %both
%query and support features.
This paper proposes to solve the problem by %introducing query features into support prototypes, 
%modeling the query-query matching: generating query prototypes to match query features,
proposing a novel query-query matching concept: use query prototypes to match query features, or in other words, use the query feature to self-support itself.
We thus call the query prototype as {\it self-support prototype} because of its self-matching property.
%and perform self-support matching between query prototype and query features, 
%which has never been explored before.
%Different from previous works where prototypes are aggregated from only support features, we propose to leverage the query feature to generate prototypes so that the query feature can self-support itself.
%Our method redefines the prototype generation from only support features to both query and support features.
Specifically, we first generate the initial mask predictions through the naive support-query matching procedure.
Based on the initial predicted query mask, we collect high-confidence query features to generate the query prototypes, which are then used to perform self-support matching with query features.
As shown in Figure~\ref{fig:teaser}, our {\em self-support module (SSM)} collects confident features of the cat head which are used to segment the entire black cat.
The rationale behind such self-support matching design is the simple Gestalt law~\cite{gestalt} in perceptual grouping:
%the inherent object consistent distinctiveness: 
pixels belonging to the same object are more similar than those to different objects. %from both semantic and appearance levels. 
%To substantiate this argument, 
%Besides,
Our model is optimized on base classes %for the object consistent distinctiveness 
to retrieve other object parts supported by object fragments, \ie,
query self-support prototypes. %self-support prototype.


%Our experiment shows such self-support prototype is much more effective to match query features compared to traditional support prototypes. 




%\fancomment{We need better connection. Because the PSBG is based on SSM}
Now, the foreground prototype can take full advantage of our self-support module, because foreground pixels share semantic commonality as aforementioned.
On the other hand,
note that the background is usually cluttered, which does not have the global semantic commonality shared among all background pixels.
Thus, rather than generating a global background prototype by aggregating all the background pixels, we propose to adaptively generate self-support background prototypes for each query pixel, by dynamically aggregating similar background pixels in the query image.
The {\em adaptive self-support background prototype (ASBP)} is motivated by the fact that separate background regions have local semantic similarity.
%Despite the effectiveness of our self-support module, we find that the background prototype does not take full advantage of our self-support module.
Finally, we propose a {\em self-support loss (SSL)} to further facilitate the self-support procedure.

\fancomment{%Our self-support method is \textbf{novel}. It fundamentally differs from other methods.
We are the first one to perform self-support matching between query prototype and query features.
As shown in Figure~\ref{fig:teaser}, %our self-support method extracts query features to generate representative self-support (query) prototypes. 
our method fundamentally differs from other support prototype generation methods, which learns from extra unlabeled images (PPNet~\cite{liu2020ppnet} and MLC~\cite{yang2021mining}) or builds various support prototype generation modules~\cite{siam2019amp,li2021adaptive,yang2020prototype} or feature priors (PFENet~\cite{tian2020prior}) based on support images.
Although PANet~\cite{wang2019panet} and CRNet~\cite{liu2020crnet} also explore query prototypes, they uses \textit{query prototypes} to match \textit{support features} as a query-support matching only for the auxiliary training.
In contrast, we perform query-query matching between \textit{query prototypes} and \textit{query features} in both training and testing stages.
}

Our self-support method significantly improves the prototype quality by alleviating %the limited coverage of intra-class variations by few-shot supports, 
the intra-class appearance discrepancy problem,
evidenced by the performance boost on multiple datasets in our experimental validation. 
Despite the simple idea, our self-support method is very effective and has various advantages, such as benefiting more from stronger backbone and more supports, producing high-confidence predictions, more robustness to weak support labels, higher generalization to other methods and higher running efficiency. We will substantiate these advantages with thorough experiments. In summary, our contributions are:
\begin{itemize}
\vspace{-0.05in}
\setlength{\itemsep}{0.5pt}
\setlength{\parsep}{0.5pt}
\setlength{\parskip}{0.5pt}
    \item We propose a brand new query-query matching concept and build a novel self-support network to solve the appearance discrepancy problem in few-shot semantic segmentation models.
    \item We propose self-support module, adaptive self-support background prototype and self-support loss to facilitate our self-support method.
    \item Our self-support method outperforms previous SOTAs by a large margin on multiple datasets with many desirable advantages.
    %\item \fancomment{other advantages of our method: no extra parameters, improve the prediction confidence, benefit more from stronger background and more support shot, robust to support noise.}
\end{itemize}

%We further propose a pointwise similarity-sensitive background prototype generation (PSBG) to handle the background clutter problem. We propose to generate background prototypes for each query pixel by dynamically aggregating similar background pixels in the query image. 
%Finally, we propose a self-support loss to further facilitate the self-support procedure.
%Our self-support technique significantly improves the prototype quality and therefore largely boost the performance on multiple datasets. \fancomment{This paragraph needs more details and motivation. We also need to highlight the self-support prototype compared to the traditional support prototype}






%Then we propose a self-support module (SSM) to collect confident query features and aggregate them into the self-support prototype to perform matching with query features.
%The rationales behind such design are two folds. Firstly, pixels belonging to the same object are more similar from both semantic and appearance levels. \fancomment{Follow CK's suggestion} Secondly, based on the object consistent distinctiveness, the model is trained on base classes to perform self-matching using self-support prototypes. 
%We find such self-support prototypes is much more effective to match query features compared to traditional support prototypes. 



%Previous methods heavily suffer the \ourproblem problem by directly matching the support prototype and query images, where the prototype is aggregated from support features with 
%In this paper, we propose to leverage the query features for support prototype generation to narrow down the feature gap between query and supports.

% 3. Our method

%Motivated by the fact that pixels belonging to the same object are more similar from both semantic and appearance levels.


%give an example to illustrate this problem. (cosine similarity between pixels of the same object, pixels and prototype of other object)
%In this work, we aim to solve this problem by ...





%Despite the success of siamese matching netowrks, there is a fundamental problem in FSS: feature gap between query and support images. It is caused by the small data volume with large data diversity which is derived from the inherent data scarcity of few-shot tasks. Most FSS works attempt to solve this problem from various aspects, e.g., matching mechanism~\cite{}, training supervision~\cite{} and support generation~\cite{}. 



%There are two fundamental problems in FSS caused by the inherent data scarcity: overfitting towards training samples and large feature gap between query  The few data causes two problem, overfitting towards a few training data, and feature gap between query and support. The former problem can be effectively solved by the prototype-based matching network through learning a class-agnostic general matching metric, which is widely adopted as the mainstream paradigm. The feature gap problem is derived from the small data volume and large data diversity. It is hard to solve and most works are trying to find the solution from various aspects, e.g., better matching method, more data and better support generation to bridge the feature gap. In this paper, we propose a simple and effective method to solve the feature gap problem: self-support matching network.

%Due to the few data, the model is easy to overfit. Therefore, the prototype-based matching network is proposed to solve the overfitting problem.
%The prototype-based matching network is  which is effective to solve the overfitting problem 

%Semantic segmentation is a fundamental problem in computer vision, where some remarkable advances have been made over the past decade tapping into the rapid development of deep learning networks~\cite{Goodfellow-et-al-2016} and large-scale datasets such as~\cite{deng2009imagenet}. However, current high-performing semantic segmentation methods rely heavily on pixel-level well-annotated training samples, and collecting such high-quality data is very expensive. 
%\fancomment{Maybe we can remove the following sentence to shorten the background.} Such massive annotated data requirement has heavily impeded the development in machine semantic understanding toward the real world, where visual objects distribution is long-tailed with numerous rare classes. This is evidenced by comparing  the large-scale classification datasets with more than 10,000 categories (OpenImage dataset with 19,957 classes), versus the most popular semantic segmentation datasets which usually contain limited classes, e.g., Pascal VOC with 20 classes, MS COCO with 80 classes and ADE20k with 150 classes. 

% 2. Introduce previous works
%\fancomment{FSL starts from 2016, isn't it new?} \ck{not quite; FF Li's 2006 PAMI on one/few shot learning when she was Caltech PhD} \fancomment{Oh, I see! FSL just becomes hot from 2016.}

%Few shot learning is not new, where researchers~\cite{shaban2017one,dong2018few} have introduced few-shot learning into semantic segmentation task to segment arbitrary novel classes using only a few support training examples. In particular, Dong et al.~\cite{dong2018few} has proposed a prototype-based matching network to address the few-shot semantic segmentation (FSS) task, which is based on the prototype theory from cognitive science~\cite{rosch1973natural} adopting from prototypical networks~\cite{snell2017prototypical} in few-shot classification. Specifically, a siamese network is first utilized to extract features for support-query image pairs. Then the support features are aggregated into support prototypes and matched with the query feature to generate the similarity map as the prediction. This procedure is class-agnostic and thus can be generalized to novel classes. Since this introduction of using siamese network, this approach has become mainstream in addressing few-shot semantic segmentation inspiring  other works~\cite{bhunia2019deep,siam2020weakly,zhu2020self,liu2020crnet,tian2020prior}.


%\ck{\cite{dong2018few} is only cited 174 times by google scholar. Still mainstream? } \fancomment{Yes, the citation is not high because FSS is an emerging task from BMVC2017 (\cite{shaban2017one} is cited by 223 times) and receive attentions from ICCV2019. }
%Shaban et al.~\cite{} first proposes %to undertake few-shot semantic segmentation (FSS) task with the leverage of a siamese network on support-query image pairs to measure their feature similarity.
%Specifically, support features are first aggregated into support prototypes and then matched with the query feature to generate the similarity map as the prediction. This procedure is class-agnostic and therefore can generalize to novel classes.
%It is the mainstream paradigm to solve few-shot semantic segmentation. %and improved by other methods from various aspects, e.g., better training strategy~\cite{}, matching metric~\cite{} and support aggregation~\cite{}.

% 2.1 support prototype to match with query feature
% mainly follow this paradigm to build the model
% 2.2 better loss and other designs
% 2.3 better support

% 2.2 some works optimize the backbone with a non-parametric metric with xxx, xxx, and xxx
% 2.3 some works directly optimize a parametric metric consisting of a couple of convolutional layers and improve the method with xxx, xxx and xxx
% 

\begin{comment}

% 3. Introduce problem
Support prototype takes an instrumental role in few-shot semantic segmentation, and thus its generation method has attracted the most attention from researchers. % We need to emphasize the significance of support generation
The basic prototype generation is using the masked average pooling operation to aggregate support features.
Many works attempt to improve the prototype generation procedure with various techniques, e.g., 
%attention mechanism~\cite{zhang2019canet}, adaptive masked proxies~\cite{siam2019amp}, pyramid attention graph~\cite{zhang2019pyramid}, prototype alignment regularization~\cite{wang2019panet}, part-aware prototype network~\cite{liu2020part}, prototype mixture models~\cite{yang2020prototype}, democratized graph attention~\cite{wang2020few}, adaptive local prototype pooling~\cite{ouyang2020self}, self-guided and cross-guided learning~\cite{zhang2021self}, adaptive prototype learning and allocation~\cite{li2021adaptive}, quality measurement~\cite{wu2021learning} and prototype rectification~\cite{yang2021mining}. \fancomment{we need to cluster them for clarity.}
attention mechanism~\cite{zhang2019canet,zhang2019pyramid,wang2020few},
%attention mechanism~\cite{zhang2019canet}, pyramid attention graph~\cite{zhang2019pyramid}, democratized graph attention~\cite{wang2020few}, 
adaptive prototype learning~\cite{siam2019amp,li2021adaptive,ouyang2020self},
%adaptive masked proxies~\cite{siam2019amp}, adaptive prototype learning and allocation~\cite{li2021adaptive}, adaptive local prototype pooling~\cite{ouyang2020self},
prototype regularization~\cite{wang2019panet,zhang2021self,yang2021mining},
%prototype alignment regularization~\cite{wang2019panet}, self-guided and cross-guided learning~\cite{zhang2021self}, and prototype rectification~\cite{yang2021mining}.
or others~\cite{liu2020part,yang2020prototype,wu2021learning}.
%part-aware prototype network~\cite{liu2020part}, prototype mixture models~\cite{yang2020prototype}, quality measurement~\cite{wu2021learning} 
Despite their success, they all focus on mining or aggregating representative prototypes only from support images.
%However, {\it should we only use support features to generate prototypes?}
However, {\it should prototypes only generated from support features?}
In this work, we investigate the prototype generation from a brand new perspective and propose %a simple yet effective prototype generation method.
a {\bf self-support prototype} aggregated from query features for effective prototype-based matching.

\end{comment}


% 4. Introduce previous solutions
%\fancomment{Should we refine the support prototype definition?}
%In previous works, support prototypes are defined and extracted from support features. However, {\it should we limit the support prototype definition only on support images?} The answer is {\bf no}. % We redefine the support prototype, it is very important because we investigate support prototype from a brand new view.
%We redefine the support prototype as follows: \fancomment{the definition is not good.}
%support prototype is extracted from image features to perform matching with query features, which can be from support or query images.

%\fancomment{another aspect: what is a good support prototype? prototype aggregated from other support images, or from the query image itself?}






%We also find such self-support based self-matching is much more effective than traditional query-support matching. \fancomment{proved by experiment} 




%Support prototype is essential for FSS and attracts the most attention from researchers. % We need to emphasize the significance of support generation
%he basic support prototype generation is using the masked average pooling operation to aggregate support features.
%PPNet~\cite{} proposes 


% 5. Introduce our solution
% 6. Summary

